Supervisory Control for Behavior Composition

We relate behavior composition, a synthesis task studied in AI, to supervisory control theory from the discrete event systems field. In particular, we show that realizing (i.e., implementing) a target behavior module (e.g., a house surveillance system) by suitably coordinating a collection of available behaviors (e.g., automatic blinds, doors, lights, cameras, etc.) amounts to imposing a supervisor onto a special discrete event system. Such a link allows us to leverage on the solid foundations and extensive work on discrete event systems, including borrowing tools and ideas from that field. As evidence of that we show how simple it is to introduce preferences in the mapped framework.

==> 5-BCpreferences.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Composition under Constraints} %\label{sec:DEScomposition-preferences}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In practical applications, it may be desirable to restrict to composition solutions conforming to some given constraints. Such constraints can pertain to the evolution of one or more available behaviors or to the way behaviors are scheduled by the controller. 
%%
For example, the designer may require that a given available behavior never reaches an internal (dangerous) state. Similarly, she may impose fairness or load balancing restrictions on how tasks are delegated to behaviors. So, under certain conditions, an action should never be delegated to the same behavior twice in a row, or at least half of the modules need to be used.
%%
Up to our knowledge, so far this has never been explored in the AI literature. We show how such constraints can be naturally accommodated in a DES-based composition framework as the one presented above.

\begin{example}\label{ex:constr} 
Consider again the setting in Figure~\ref{fig:ambientIntel-system}. 
%%
Assume the additional requirement that, whenever the excavator is ``improperly'' used for loading, it is then the first vehicle to be repaired (for instance, because it is the most vulnerable to wear, and late repairs are expensive). 
%%
By inspection of the solution in Figure~\ref{ex:CG}, it is easy to see that such solution exists, and it amounts to removing all states $x\geq 12$  from $\CGDES$ (i.e., use $\B_3$ ``only if strictly necessary'').
\end{example}

In order to represent behavior composition under constraints, we consider the extended problem of computing a composition $\Comp$ for a target $\Targ$ on a system $\S$ \emph{under a constraint specification language $\C \subseteq \H$}. Informally, controller $\Comp$ is meant to generate  system histories inside $\C$.
 


\begin{figure}[b!]
\begin{center}
\resizebox{\columnwidth}{!}{\input{fig-cg-mining-constr}}
% \vspace{-.25in}
\caption{$\CGDES$ for Example~\ref{ex:constr} under the constraint language $\CSpec  = 
	\set{ w \mid w = w_1 \concat \aload \concat 3 \concat w_2
          \concat \arepair \concat 3 \concat w_3, \text{ with }  w_1,w_3 \in \Sigma^*, 
				w_2 \in (\Sigma\setminus \set{\arepair})^*}$. 
%%
Module $\B_3$ is used to load ``only if necessary'' (see state $2$, reachable by a nondeterministic transition of $\B_1$).}
\label{ex:CG-constr}
\end{center}
% \vspace{-.25in}
\end{figure}


\begin{definition}
A controller $\Comp$ \defterm{conforms} to constraints $\C \subseteq \H$ iff $\H_{\Comp,\tau} \subseteq \C$, for any target trace $\tau$.  
\end{definition}

In other words, $\Comp$ conforms to $\C$ iff the executions it induces, when running the target, yield constraint-compatible histories.
%%
Note that this setting is strictly more expressive than the standard composition task, as the constraints' alphabet may go beyond target actions (e.g., it can also mention behavior delegations and internal states of the available behaviors). 
%%
Of course, $\C = \H$ yields the classical setting (i.e., no constraints).
 
So, to solve a (constrained) composition problem using our DES-based approach, we first map the constraint specification $\C$ to its DES version by taking 
\[
	\CSpec = \set{\word^{-1}(h) \mid h \in \C}.
\]
%%
Observe that $\CSpec \subseteq \Act^*$ (where $\Sigma$ is the set of events of the composition plant $\Plant$), even though, of course, at most the regular language $\CSpec \cap \Mkd(\Plant)$ can be controlled.
%%
We require the set $\C$ to be prefix-closed, that is, if a history $h$
belongs to $\C$ so do all its prefixes.

Finally, we just apply the approach from the previous section, now using $\CSpec$ directly as the specification of the language to be controlled.
%% 
Note that if $\Mkd(\Plant)\subseteq\CSpec$---everything that the plant may generate is constraint-compatible---then $\CSpec$ plays no role and the problem reduces to the standard constraint-free setting.
%%
On the other hand, when $\Mkd(\Plant) \setminus \CSpec \not= \emptyset$, any composition solution may be inadequate.


Since $\C$ is a prefix-closed set of histories, language $\CSpec$ is closed as well, that is, $\CSpec =
\Closure{\CSpec}$. As a consequence, we have $\Closure{\CSpec} \cap \Mkd(\Plant) \subseteq \CSpec$.
%%
Hence, from Theorem~\ref{theo:supNSC}, we conclude that if $\supremal{\CSpec} \neq\emptyset$, then there exists a nonblocking supervisor $\sup$ for $\Plant$ with $\Mkd(\sup/\Plant) = \supremal{\CSpec} = \Closure{\supremal{\CSpec}}$.
%%
%%
Figure \ref{ex:CG-constr} shows the DES controller generator for Example~\ref{ex:constr}.
%
This leads us to the main result of this section.




\begin{theorem}[Soundness]
There exists a nonblocking supervisor $\sup$ such that
$\Mkd(\sup/\Plant)=\supremal{\CSpec}\neq\emptyset$ iff there exists a
controller $\Comp_\sup$, induced by $\sup$, that is a composition for
target $\Targ$ in system $\S$ conforming to $\C$.
\end{theorem}

\begin{proof}
$(\Rightarrow)$ Assume by contradiction that $\sup$ is such that $\Mkd(\sup/\Plant)=\supremal{\CSpec}\neq\emptyset$ but for some target trace $\tau$ and history $h\in\H_{\Comp,\tau}$ there exists a controller $\Comp_\sup$ induced by $\sup$ such that either $(1)$ it is not a composition or $(2)$ $\Comp_\sup(h,\sigma_{\Card{\tau}})=j$ but $\word(h)\concat \sigma_{\Card{\tau}} \concat j\not\in\CSpec$.
%%
Case $(2)$ is contradictory because $\Comp_\sup(h,\sigma_{\Card{\tau}})=j$ implies that $j\in\sup(\word(h),\sigma_{\Card{\tau}})$, and hence it can not be the case that $\word(h)\concat \sigma_{\Card{\tau}} \concat j\not\in\CSpec$, since $\Mkd(\sup/\Plant)=\supremal{\CSpec}$.
%%
As for $(1)$, we can easily follow the same reasoning as for Theorem~\ref{theo:soundness}.
%%
%%

$(\Leftarrow)$ 
%
By Lemma~\ref{lemma:final} we have that $\Comp_\sup$ is such that, for each history $h\in \H_{\Comp_\sup,\tau}$,
$\word(h)\in \supremal{\Specc}$. If then $\supremal{\CSpec}=\emptyset$
it means that $\word(h)\not\in \supremal{\CSpec}$. However, this
contradicts the fact that $h\in\C$, thus $\Comp_\sup$ does not conform
to $\C$.
%%
%%
%%
 \end{proof}

\begin{theorem}[Completeness]
Given a nonblocking supervisor $\sup$ such that $\Mkd(\sup/\Plant)=\supremal{\CSpec}$, every composition $\Comp$ for target
$\Targ$ in system $\S$ conforming to $\C$ is induced by $\sup$.
%%
\begin{proof}
Assume by contradiction that there exists a composition $\Comp'$ for
$\Targ$ in 
$\S$ conforming to $\C$ that can not be induced by a supervisor $\sup$ as above. This means that for some target trace $\tau$ and some system history $h\in\H_{\Comp,\tau}$ we have $\Comp'(h,\sigma_{\card{\tau}}) \not\in \sup(h,\sigma_{\card{\tau}})$.
%%
The proof thus proceeds as for Theorem~\ref{theo:completness} to
exclude that 
%%
$(1)$ $\word(h)\concat \sigma_{\card{\tau}}\not\in \Gtd(\Plant)$, i.e., action $\sigma_{\card{\tau}}$ is not available from target state $\stateproj_t(last(h))$ or $(2)$ $\word(h)\concat \sigma_{\card{\tau}} \concat j \not\in \Gtd(\Plant)$, i.e., behavior $\Be{j}$ can not perform such an action from its state $\stateproj_j(last(h))$ or $(3)$ for all words $w\in\Mkd(\Plant)$ with $w>\word(h) \concat \sigma_{\card{\tau}} \concat j$ we have $w\not\in\CSpec$.
%%
All these cases imply that $\Comp'$ is not a composition. 
It remains to show that $(4)$ if
$\Comp'(h,\sigma_{\card{\tau}})=j$ then $\word(h)\concat
\sigma_{\card{\tau}}\concat j \in \Closure{\C}$. This contradicts the
fact that $\Comp'$ conforms to $\C$.
\end{proof}
\end{theorem}

As before, once we have a supervisor $\sup$ as in the above theorems, one can reconstruct all composition controllers $\Comp$ conforming
with $\C$.
%%
In turn, assuming regularity of constraint specification $\C$, we can finitely implement the supervisor with a generator $\R$ as in the previous section.
%%
However, the procedure for building the DES controller generator from $\R$ needs to be adapted, as we need more information than the current state of the behaviors and the target.
%%
More concretely, generator $\R$ may require additional bounded memory to witness the satisfaction of constraints. For example, we can build a specification $\CSpec'$ for Example~\ref{ex:constr}, in which we constrain the controller to alternate the delegation of action $\aload$ to $\B_2$ and $\B_3$, or to use $\B_3$ only a fixed number of delegations to $\B_2$ first. It is easy to notice that all these examples require an additional amount of memory.
%

\begin{definition}
Therefore, given the automaton $\R$, we define the \defterm{\emph{memory-based} DES controller generator} $\CGDESMEM = \tup{\Act_t,\Services,Q',  q'_0,\vartheta',\omega'}$ as before, except that the state space $Q'$ is just a subset of $\R$'s state set $Y$, namely, 
$Q' = \set{y\in Y \mid  p\in(\Act_t \concat \Services\concat \Nondet)^*, y = \rho(y_0,p)}$. 
\end{definition}




Summarizing, the fact that supervisory control theory is based entirely on languages allows us to integrate sophisticated constraints for the composition task in an almost straightforward manner, by just seeing constraints as sets of ``allowed'' words that the composition plant may generate.


\endinput


